TLXML: Task-Level Explanation of Meta-Learning via Influence Functions

Meta-learning enables models to rapidly adapt to new tasks by leveraging prior experience, but its adaptation mechanisms remain opaque, especially regarding how past training tasks influence future predictions. We introduce TLXML (Task-Level eXplanation of Meta-Learning), a novel framework that extends influence functions to meta-learning settings and provides task-level explanations of adaptation and inference. By reformulating influence functions for the bi-level structure of meta-learning, we quantify the contribution of each meta-training task to the adapted model's behaviour. To ensure scalability, we propose a Gauss-Newton-based approximation that significantly reduces computational complexity from $O(pq^2)$ to $O(pq)$, where $p$ and $q$ denote the numbers of model and meta parameters, respectively. Moreover, we propose generalized influence functions defined using pseudo-inverse Hessian, which are applicable even when the loss landscape has flat directions. Results demonstrate that TLXML effectively ranks training tasks by their influence on downstream performance, offering concise, intuitive explanations aligned with user-level abstraction. This work provides a critical step toward interpretable and trustworthy meta-learning systems.

==> table/noise_distinction/digest.tex <==
\begin{table}
\centering
\caption{
Experiment of distinguishing noise tasks and normal task distributions.
MI and OM represent MiniImagenet and Omniglot respectively. The standard deviation $\sigma$ under the hypothesis of the random ordering is $\sqrt{0.5\times 0.5 \times 128} \sim 5.66$. 
$\pm$ means the average and standard deviation across 5 runs of training.
}
\label{tab: noise_distinction_small}
\begin{tabular}{cccc}
\toprule
Meta-learner & Dataset & \multicolumn{2}{c}{Proper tests} \\
             {} &      {} & [count] &            [$\sigma$] \\
\midrule
           MAML &      MI & 85.6$\pm$11.1 &  3.8$\pm$2.0 $\sigma$ \\
           MAML &      OM &  94.0$\pm$6.0 & 5.3$\pm$1.1 $\sigma$ \\
       Protonet &      MI &  95.6$\pm$5.3 &  5.6$\pm$0.9 $\sigma$ \\
       Protonet &      OM &  81.2$\pm$5.5 &  3.0$\pm$1.0 $\sigma$ \\
\bottomrule
\end{tabular}
\end{table}
